GraphQ IR: Unifying the Semantic Parsing of Graph Query Languages with One Intermediate Representation

Subject to the huge semantic gap between natural and formal languages, neural semantic parsing is typically bottlenecked by its complexity of dealing with both input semantics and output syntax. Recent works have proposed several forms of supplementary supervision but none is generalized across multiple formal languages. This paper proposes a unified intermediate representation (IR) for graph query languages, named GraphQ IR. It has a natural-language-like expression that bridges the semantic gap and formally defined syntax that maintains the graph structure. Therefore, a neural semantic parser can more precisely convert user queries into GraphQ IR, which can be later losslessly compiled into various downstream graph query languages. Extensive experiments on several benchmarks including KQA Pro, Overnight, GrailQA, and MetaQA-Cypher under standard i.i.d., out-of-distribution, and low-resource settings validate GraphQ IR's superiority over the previous state-of-the-arts with a maximum 11% accuracy improvement.

==> sections/tab_grammar.tex <==
\begin{table*}[t!]
\centering
\small
\resizebox{\textwidth}{!}{
\begin{tabular}{p{0.175\textwidth}>{\raggedright}p{0.55\textwidth}>{\raggedright\arraybackslash}p{0.3\textwidth}}
\toprule
\textbf{Non-terminal} & \textbf{Productions} & \textbf{Description} \\
\midrule
$S$ &$\rightarrow$ \texttt{EntityQuery} | \texttt{AttributeQuery} | \texttt{RelationQuery} |  \texttt{QualifierQuery} | \texttt{ValueQuery} | \texttt{CountQuery} & Start symbol of a query sequence \\
\hline
\texttt{EntityQuery} &$\rightarrow$  \textit{what is} \texttt{EntitySet} & Query that returns certain entities \\
\hline
\texttt{RelationQuery} &$\rightarrow$ \textit{what is the relation from} \texttt{EntitySet} \textit{to} \texttt{EntitySet} & Query that returns the relationship between given entities \\
\hline
\texttt{CountQuery} &$\rightarrow$  \textit{how many} \texttt{EntitySet} & Query that returns the quantity of certain entities \\
\hline
\texttt{EntitySet} &$\rightarrow$ \texttt{<ES> EntitySet LOP EntitySet </ES>} | \texttt{<ES>} \texttt{EntitySet Constraint} \texttt{</ES>} | \texttt{Concept} | \texttt{Entity} & A non-empty set of entities that match certain conditions \\
\hline
\texttt{Constraint} &$\rightarrow$ \textit{whose} \texttt{Attribute COP Value} | \textit{that} \texttt{Relation DIR} \textit{to} \texttt{EntitySet} | \textit{that} \texttt{Relation DIR} \textit{to} \texttt{COP} \texttt{Value} \texttt{EntitySet} & Clauses that constrain the entities condition \\
\hline
\texttt{Entity} &$\rightarrow$ \texttt{<E>} \textit{entity} \texttt{</E>} & Entity node of a specified name \\
\hline
\texttt{Concept} &$\rightarrow$ \texttt{<C>} \textit{concept} \texttt{</C>} & Set of entities of a specified type\\
\hline
\texttt{Attribute} &$\rightarrow$ \texttt{<A>} \textit{attribute} \texttt{</A>} & Specified property of an entity  \\
\hline
\texttt{Relation} &$\rightarrow$ \texttt{<R>} \textit{relation} \texttt{</R>} & Relationship between entities \\
\hline
\texttt{Value} &$\rightarrow$ \texttt{VTYPE <V>} \textit{value} \texttt{</V>} | \texttt{Attribute} \textit{of} \texttt{Entity} & Specified value of certain constraints \\
\hline
\texttt{LOP} &$\rightarrow$ \textit{and} | \textit{or} | \textit{not} & Logical operators that perform set union, intersection or exclusion \\
\hline
\texttt{COP} &$\rightarrow$ \textit{is} | \textit{is not} | \textit{larger than} | \textit{smaller than} | \textit{at least} | \textit{at most} & Comparison operators that take value as operand \\
\hline
\texttt{DIR} &$\rightarrow$ \textit{forward} | \textit{backward} & Relationship direction constraint \\
\hline
\texttt{VTYPE} &$\rightarrow$ \textit{string} | \textit{number} | \textit{year} | \textit{date} | \textit{time}  & Value type constraint \\
\bottomrule
\end{tabular}
} 
\caption{A subset of \tool grammar rules. We separate alternative productions at the same level using ``|'' and mark the terminal nodes in italics. A more complete set of grammar is presented in Appendix Table \ref{tab:full_grammar}. }
\label{tab:grammar}
\end{table*}
